Optimal Trajectories of a UAV Base Station Using Hamilton-Jacobi Equations

We consider the problem of optimizing the trajectory of an Unmanned Aerial Vehicle (UAV). Assuming a traffic intensity map of users to be served, the UAV must travel from a given initial location to a final position within a given duration and serves the traffic on its way. The problem consists in finding the optimal trajectory that minimizes a certain cost depending on the velocity and on the amount of served traffic. We formulate the problem using the framework of Lagrangian mechanics. We derive closed-form formulas for the optimal trajectory when the traffic intensity is quadratic (single-phase) using Hamilton-Jacobi equations. When the traffic intensity is bi-phase, i.e. made of two quadratics, we provide necessary conditions of optimality that allow us to propose a gradient-based algorithm and a new algorithm based on the linear control properties of the quadratic model. These two solutions are of very low complexity because they rely on fast convergence numerical schemes and closed form formulas. These two approaches return a trajectory satisfying the necessary conditions of optimality. At last, we propose a data processing procedure based on a modified K-means algorithm to derive a bi-phase model and an optimal trajectory simulation from real traffic data.

==> Optimal UAV trajectory using HJB/alternating-descent-algorithm.tex <==
% alternating-descent-algorithm.tex
% ms 21.09.20

\subsection{An Alternating Optimization Algorithm}

We now study a time-independent bi-phase scenario, in which a trajectory from $z_0$ to $z_T$ crosses the interface at time $\tau$ and location $\xi$. We present an Alternating Optimization Algorithm (Algorithm~\ref{alg:aoa}) that provides a stationary trajectory in the sense of Theorem~\ref{th:multiphase}. The algorithm consists in alternatively optimizing $\tau$ (steps 9-17) and $\xi$ (steps 18-26) by using the results of Theorem~\ref{th:multiphase}. For every fixed $\tau$ and $\xi$, the current trajectory is the concatenation of the optimal trajectory between $(t_0,z_0)$ and $(\tau,\xi)$ and the optimal trajectory between $(\tau,\xi)$ and $(T,z_T)$ (step 27). Every iteration of the algorithm only requires the evaluation of two Hamiltonians or the computation of a point $B$, see \eqref{location-B-ms:eq}, and its projection on the interface. Therefore the complexity of an iteration is  $O(1)$. In simulations, MPC is used to produce an initial trajectory.

\def\HSPONE{z_{h1}} % HOTSPOT 1
\def\HSPTWO{z_{h2}} % HOTSPOT 2

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.8\linewidth]{mpc-vs-aoa}
\end{center}
\caption{\label{fig:mpc-vs-aoa}MPC trajectory and Alternating Optimization Algorithm trajectory with two hot spots.}
\end{figure} 

\begin{figure}[H]
\begin{center}
\includegraphics[width=0.8\linewidth]{costfunction-scenario4}
\end{center}
\caption{\label{fig:costfunction-tau-scenario4}Cost function along the iterations of the Alternating Optimization Algorithm trajectory.}
\end{figure}



MPC
This projection is performed in steps 19-20 of the algorithm.


Figure~\ref{fig:mpc-vs-aoa} shows the MPC trajectory and the trajectory obtained from Algorithm~\ref{alg:aoa} after 60 iterations in a bi-phase landscape. The traffic intensity is shown in three dimensions in Figure~\ref{fig:systemmodel}: It is a bi-phase landscape made of two hot-spots, where the peak of traffic in $z_{h2}$ is higher than in $z_{h1}$. The Alternating Optimization Algorithm has gradually moved the interface crossing time and location in order to spend more time in the second hot-spot and to go closer to $z_{h2}$. 
Figure~\ref{fig:costfunction-tau-scenario4} shows how the cost function has decreased along the iterations and thus how our algorithm has improved over the MPC solution. From iterations 1 to 45, $\tau$ has been gradually updated; at iteration 46, $\xi$ is updated once; $\xi$ is again updated once at iteration 59.
%
\begin{comment}
In Figure~\ref{fig:potentialenergy-speed-scenario4} (top), we see how the difference between the potential energy before and after the interface tends to zero. Figure~\ref{fig:potentialenergy-speed-scenario4} (bottom) shows the difference between the velocity vectors before and after crossing the interface. On the resulting stationary trajectory, velocity is continuous on the interface.  
\end{comment}



\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%
\begin{algorithm}%[H]
\caption{Alternating Optimization Algorithm}\label{alg:aoa}
\begin{algorithmic}[1]
\State {\bf Input:} $t_0$, $T$, $z_0$, $z_T$, $z_{h1}$, $z_{h2}$, $u_{01}$, $u_{02}$, $\omega_1$, $\omega_2$, $u_{11}$,  $u_{12}$, an initial trajectory $z(t)$, the initial crossing time and position $(\tau, \xi)\in [\tau;T]\times \mathcal{I}$, $\delta \tau>0$, $\epsilon_{\tau}>0$, $\epsilon_{\xi}>0$, $\epsilon_{S}>0$.
\State {\bf Output:} $(\tau, \xi)\in [\tau;T]\times \mathcal{I}$  such that the conditions of Theorem~\ref{th:multiphase}
\State $\tau'\gets \tau$; $\xi'\gets \xi$
\State $\texttt{timenotfound} \gets 1$; $\texttt{positionnotfound} \gets 0$
\State $\{z(t)\}_{t_0\leq t\leq T}\gets $ an initial feasible trajectory, e.g. from MPC
\State Compute $S$ along $\{z(t)\}_{t_0\leq t\leq T}$
\Do
	\State $S'\gets S$
	\If{$\texttt{timenotfound}$}
		\State Compute $H_1$ and $H_2$ at $(\tau, \xi)$ according to (\ref{Hamilton-Jacobi-backward-ms:eq}-\ref{Hamilton-Jacobi-forward-ms:eq})
		\State $\tau \gets \tau + sign(H_1-H_2)\delta \tau$
		\If{$|\tau'-\tau|<\epsilon_{\tau}$}
			\State $\texttt{timenotfound}\gets 0$
			\State $\texttt{positionnotfound} \gets 1$
		\EndIf
		\State $\tau'\gets \tau$
	\EndIf
	\If{$\texttt{positionnotfound}$}
		\State Compute $B$ according to (\ref{location-B-ms:eq})
		\State $\xi \gets proj_{\mathcal{I}}(B)$, see (\ref{algo-proj-B:eq}) %$\nabla_{\xi} S=h(\xi-B)$
		\If{$||\xi'-\xi||<\epsilon_{\xi}$}
			\State $\texttt{timenotfound}\gets 1$
			\State $\texttt{positionnotfound} \gets 0$
		\EndIf
		\State $\xi'\gets \xi$
	\EndIf
    \State $\{z(t)\}_{t_0\leq t \leq T}\gets \texttt{OPTTRAJ}(z_{h1}, u_{01}, u_{11}, \omega_1, z_0, t_0,$ $\xi, \tau) \cup \texttt{OPTTRAJ}(z_{h2}, u_{02}, u_{12}, \omega_2, \xi, \tau, z_T, T)$  (\texttt{OPTTRAJ} provides optimal trajectory using \eqref{eq:trajhotspot},\eqref{eq:ellipse})
    %see \texttt{OPTTRAJ} function in Algorithm~\ref{alg:mpc})
    \State Cd{comment}ompute $S$ for $\{z(t)\}_{t_0\leq t\leq T}$ according to (\ref{eq:vu0neg}) 
\doWhile{$|S'-S|>\epsilon_S$}
\end{algorithmic}
\end{algorithm}



\begin{comment}
\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{potentialenergy-speed-scenario4v2}
\end{center}
\caption{\label{fig:potentialenergy-speed-scenario4}Alternating Optimization Algorithm trajectory: (top) $H_1-H_2$: Difference in potential energy before and after crossing the interface; (bottom) $||a_1-a_2||$: Norm of the difference of velocity vectors before and after crossing the interface.}
\end{figure}
\end{comment}

==> Optimal UAV trajectory using HJB/gradient-convergence.tex <==
% gradient-convergence.tex
%% to insert in 
%\section{Algoritms}
%\paragraph{Procedure for seeking an optimal $\tau$ given a fixed  $\xi$}
%\\
However
the following "non-convergence" results hold \textcolor{red}{MC: on a supposé que le drone traversait l'interface entre t0 et T non ? Sinon on se ramène au cas d'une seule interface, non ?}
%%%%
\begin{lemma}
\label{lem:outside-time-limits}
\eqref{h-coefficient:eq}:
Consider
$g(\tau)$ in ..
%\omega_1\, \coth(\omega_1(\tau -t_0)) + \omega_2\, \coth(\omega_2(T - \tau))$
Then
\\
%\begin{itemize}
%\item
in the case where 
$\omega_2 > \omega_1$ % check
then
$g(\tau)$ is {\bf negative} for $\tau > T$
(and also in $[t_0 - \epsilon, t_0[$)
%\item
\\
in the case where 
$\omega_1 > \omega_2$ % check
then
$g(\tau)$ is {\bf negative} for $\tau < t_0$
((and also in $]T, T + \epsilon]$)
%\end{itemize}
\end{lemma}
Proof: easy.
%\\
Thus if $\tau \notin ]t_0, T[$
the total value function could be non-convex. %% TO CHECK

\begin{theorem}
\label{th:gradient-non-convergence}
Consider current time value
$\tau \in ]t_0, T[$
and total Hessian
\eqref{eq:Hessian-second}.
%of the value function.
%\eqref{eq:Hessian-second}.
Then
\begin{itemize}
%
\item
the locus of points $\xi$
such that 
$\alpha 
= {\cal H}_{33}(\xi, \tau)
= \frac{d^2S}{d\tau^2}
< 0$
%in 
%\eqref{eq:Hessian-second}
%of the value function
is either empty
or a {\bf disk}
(inside of a {\bf circle})
\item the locus of points
such that
$\det({\cal H}(\xi, \tau)) < 0$
is either empty
or 
a {\bf disk}
%% the inside of a {\bf circle}
%
%% NOT SURE HERE-> CHECK
\begin{comment}
\item  
now consider time updating %%$\tau$:
$\tau \ra \tau + \delta \tau$ by a standard Newton-type method.
\\
%Then 
The locus of points $\xi$ such that
$\tau + \delta \tau 
\notin\ ]t_0, T[$
is the intersection two {\bf disks}
(possibly empty)
%either empty or a {\bf circular crown}
\end{comment}
%%
\end{itemize}
\end{theorem}
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Proof in Appendix
\ref{app:gradient-non-convergence-proof}
%%% PROOFS  %
\input{proof-gradient.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% RESULTS %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\\[1mm]
Influence of initial time $\tau_0$
associated "non-convergence basin" of starting points
$\xi_0$
in the \GRADALGO
are shown in in Figs
\ref{fig:marceau-non-convex1}
and
\ref{fig:marceau-non-convex2}.
%\\
In this example,
$z_T = (111.07, 13.164)$
%yielding
,
$szT = (77.78, 182.22)$ 
.
We select
$K=20, T = 800$
and the \BALGO optimal solution is 
$\xi^* = (56.65, 192.35)$ 
and 
$\tau^* = 683.15$
\enspace.

%%%%%%%%%%%%%%%%%%%
%%% FIGURES %%%%
%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\begin{subfigure}[t]{0.5\textwidth}
\centering
%
\includegraphics[width=1.\textwidth]{tau600-K20-T800.pdf}
\caption{$\tau = 600$
(close to solution) }
\label{fig:marceau-non-convex1}
\end{subfigure}
%
%~
\begin{subfigure}[t]
{0.5\textwidth}
\centering
\includegraphics[width=1.\textwidth]{tau400-K20-T800.pdf}
\caption{$\tau = 400$ 
(far from solution) }
\label{fig:marceau-non-convex2}
\end{subfigure}
%\caption{test}
\caption{
%$K = 20 - T = 800$%
Each subfigure 
shows spatial non-convergence basins for $\xi$
,
for two values of $\tau$.
}
\end{figure}




==> Optimal UAV trajectory using HJB/marc-macros.tex <==
% marc-macros.tex
\def\wrt{\mbox{wrt. \,}}
\def\resp{\mbox{ resp. }}

\def\ra{\rightarrow}
\def\Ra{\Rightarrow}

%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%% NEW 01.01.21 %%% JDMS %%%%%%%%
\def\Xone{X_1}
\def\Tone{T_1}
\def\Xtwo{X_2}
\def\Ttwo{T_2}

%%%
\def\Pone{\nabla_{\Xone}}
\def\Ptwo{\nabla_{\Xtwo}}
%5
\def\Hone#1{\dpart{#1}{\Tone}} % \Hone{S)(A,B,C,D)
\def\Htwo#1{\dpart{#1}{\Ttwo}} % \Hone{S)(A,B,C,D)

%%%%%%%% NEW %%%%%%%%%%%%%%%%%%%%%

\def\xx{x} 			% -> or  z 
\def\indexone{1} 	% -> or 0
\def\indextwo{2}	 % -> or T

\def\xone{{\xx}_\indexone}
\def\xtwo{{\xx}_\indextwo}

\def\pp{p}
\def\pone{{\pp}_\indexone}
\def\ptwo{{\pp}_\indextwo}

\def\tt{t}
\def\tone{\tt_\indexone} % or 0
\def\ttwo{\tt_\indextwo} % or T

\def\w{\omega}
\def\phase{\Phi}
\def\phase{\phi}
\def\pseudop{}

%\def\transp#1{{#1}^{t}}
\def\transp#1{{#1}^{\dagger}}

\def\norm#1{\parallel {#1} \parallel}

% \trivec %%%%
\def\trivec#1#2{
\Big(
\begin{array}{c}
{%\vec
{#1}} %new
\\[-2mm] 
%{\tiny -}
\rule{2pt}{0.1pt} %[1pt]{0.2pt}
\\[-1.5mm] 
{%\vec
{#2}} %new
\end{array} \Big)}

\def\trivec#1#2{({#1},\,{#2})} % Jerome notations in the introduction

\def\dpart#1#2{\dfrac{\partial {#1}}{\partial {#2}}}
\def\dapart#1#2{\dfrac{\partial}{\partial #2} {#1}}
\def\ddpart#1#2{\dfrac{\partial^2 {#1}}{\partial {#2}^2}}
\def\dddpart#1#2#3{\dfrac{\partial^2 {#1}}{\partial {#2} \partial {#3}}}

\def\del{\delta\,}

\def\dtime#1{\dot{#1}} 
\def\ddtime{\dfrac{\mbox{d}}{\mbox{dt}}\, }
%%%%%%
\def\myS{S(\tone, \xone, \ttwo, \xtwo)} % CHECK
\def\Id{\mbox{Id}}
\def\Real{\bR} % marceau {\mathbold{R}}

\def\GRADALGO{\mbox {\textsc{Grad-Algo} }}
\def\BALGO{\mbox {\textsc{B-Algo}}}

\def\HSPONE{z_{h1}}
\def\HSPTWO{z_{h2}}

%% old version -> S(z,t)
% \hessian{\alpha}{K g }{\pi}
\def\hessian#1#2#3{
%\left[
\left(
\begin{array}{c | l}
%\\[-1mm]
#2\ \Id_2 
&
\hspace*{2mm} 
#3 %\Pi
\\[1mm]
\hline
%\\
#3^t %\transp{\Pi}
&
\hspace*{4mm}
#1
\end{array}
%\right]
\right)
}

%% new version -> S(t, z)
%\Hessian{\alpha}{K g }{\pi}
\def\Hessian#1#2#3{
\left(%[
\begin{array}{l | c}
%\\[-1mm]
#1
&
\hspace*{2mm} 
\transp{#3} %\Pi^t
\\[1mm]
\hline
%\\
#3 %\Pi
&
\hspace*{4mm}
#2\ \Id_2 
\end{array}
\right)%]
}

%%
\def\Vmean{\bar{V}}

==> Optimal UAV trajectory using HJB/marc-simus.tex <==
% marc-simus.tex

Drone initial conditions 
as well as
network simulation parameters are shown in
Table \ref{parameters:table}.
%\\
\begin{table}[h!]
\[
\begin{array}{| c c c c  | c c c c | c c c c |}
% 14 items
\hline
\multicolumn{4}{| c |}{\mbox{general}}
& % test !!
\multicolumn{4}{c |}{\mbox{zone 1}} % ok !!
&
\multicolumn{4}{c|}{\mbox{zone 2}}
\\
\hline
z_0 & z_T 
%& z_{h1} & z_{h2} 
& t_0 & T  
%%
& z_h & u_0 & u_1 & \w
%
& z_h & u_0 & u_1 & \w
%%%%%
\\ 
\hline
\hline
%%%%%% CONVEX CASE %%%%%%%%%
\multicolumn{12}{| c |}{convex\ case}
\\
\hline
%%% numerical values %%%
-1\ -1 & 10\ 10 %& 5\ 1 & 6\ 8.5 
& 0 & 2.2
%%
& 5\ 1 & 2.645 & 20 & 1.627
%
& 6\ 8.5 &  8.265 & 40 & 2.875
%%%%%
\\
\hline
\hline
%%%%%% NON-CONVEX CASE %%%%%%%%%
\multicolumn{12}{| c |}{non-convex\ case}
\\
\hline
10\ 5 & 10\ 6 
%& z_{h1} & z_{h2} 
& 0 & 3.6 
%%
& 2\ -2  & 1.6327 & 20 & 1.2778
%
& 8\ 12 &  5.102 & 40  & 2.2588
\\
\hline
\end{array}
\]
\caption{Parameters used in 
experimental simulations.
$K = 1$ for all cases
\label{parameters:table}}
\end{table}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
Results are shown in Table \ref{results-grad-b-curve:table}.
%\\
%%%%%%%%%%%%%% TABLES SOLUTIONS %%%%%%%%%%%%
\begin{table}[h]%!] %% [h!] [h]ere overrides All other options
\[
\begin{array}{|c c c c c c c c | l l |}
\hline
\multicolumn{10}{|c|}
{\mbox{\em convex case}}
\\
\hline
%%
\xi & \norm{p^+ - p^-} & \hat{S} 
& |{\cal H}|
& H^+ & H^-  
& \tau &  T
& \mbox{ Solution} 
& % new
%%%%%%%%%%%%%%% CONVEX CASE %%%%%%%%%%%%%%%%%%%
\\[3mm]
\hline
\hline
 4.8481~5.3883 & 0.00981
& \mathbf{33.096 } 
& +
& 44.797  & 44.797  &  0.964  &   2.2
&
\GRADALGO
& % new
Fig.\ \ref{fig:convex-solution}
%%
\\[3mm]
\hline 
4.8456~5.3888 & 0.00000
& 33.096 
& +
&  44.801  & 44.797 & 0.9637 & 2.2
&
\BALGO & '' % new
%%%%%%%%%%%%%%%% NON-CONVEX CASE %%%%%%%%%%%%%%
\\[3mm]
\hline
\hline
\multicolumn{10}{|c|}
{\mbox{\em non-convex case}}
\\
\hline
6.3726~6.2484 & 0.00320 
& 100.32 
& -
& 10.773  & 10.773  & 2.6773  & 3.6
&
\mbox{n. 1 } \GRADALGO
&
Fig.\ \ref{fig:non-convex-1st-solution}
%%%%%
\\[3mm]
6.3733~6.2482 & 0.00000
& 100.32
& -
& 10.771  & 10.775 &  2.6771  &  3.6
&
\mbox{n. 1 } \BALGO
&
%[a,b]=[1,3]
''
%%%%%
\\[3mm]
9.8461~5.5062 & 0.0000
& \mathbf{-39.416} 
& +
& 39.881 & 39.862 & 0.035  & 3.6
& 
\mbox{n. 2 }\BALGO 
%% THE GOOD ONE !!
&
Fig.\ \ref{fig:non-convex-2nd-solution}
%%%%%
\\[3mm]
%\hline 
6.3302~6.3865 &  0.00180
& 78.338 
& +
&  16.123 &  16.123 & 3.5462  & 3.6
&
\mbox{n. 3 } \BALGO
&
Fig.\ \ref{fig:non-convex-3rd-solution}
\\[1mm]
\hline
%%%%%%%%%%%%%
\end{array}
\]
%%
\caption{\label{results-grad-b-curve:table}
Table of results with both gradient and the $B-$curve algorithms}
\end{table}
%%%%%%%
%~\\
Some remarks on the results:
\begin{enumerate}
\item the \GRADALGO and the dichotomic \BALGO 
with initial search interval
$[a, b] = [t_0, T]$
coincide
to the same %numerical 
optimum $(\xi^*, \tau^*)$ 
for the {\em convex} simulation case
(less that $3.\ e^-3$ on $\tau^*$)
\enspace.
%%
\item the \GRADALGO and the dichotomic \BALGO 
with initial search interval
$[a, b] = [1.,3.]$)
coincide
to the same %numerical 
optimum $(\xi^*, \tau^*)$ 
for the {\em non-convex} simulation case: 
(about $2.\ e^-4$ on $\tau^*$)
\enspace.
%
\item 
The two other (local) optimal solutions for this non-convex case
(including the global optimum, namely  $\#2$) are only attained by the \BALGO.
\item a note on local eigenvalues sign
: possible non-convexity (saddle point)
\end{enumerate}
%%
%%%%%%%%%%%%%% FIGURES SOLUTIONS %%%%%%%%%%%%
\begin{figure}[h!] %% [h!] [h]ere overrides All other options ?
\begin{center}
\subcaptionbox{\label{fig:convex-solution}
{\em convex case} (short time)  solution \GRADALGO}
{\includegraphics[width=0.65\linewidth,height=0.65\linewidth]{convex-case-solution.pdf}}
%%
\subcaptionbox{\label{fig:non-convex-1st-solution}
{\em non convex} (long time) 1st solution \GRADALGO}
{\includegraphics[width=0.65\linewidth,height=0.65\linewidth]{non-convex-1st-solution.pdf}}
\end{center}
%\caption{
\end{figure}
%%%%%%%%%%%
%%%%%%%%%%
\begin{figure}[h!] %% [h!] [h]ere overrides All other options ?
\begin{center}
\subcaptionbox{\label{fig:non-convex-2nd-solution}
{\em non convex} (long time) {\bf 2nd solution} algo-B .}
{\includegraphics[width=0.65\linewidth,height=0.65\linewidth]{non-convex-2nd-solution.pdf}}
%%
\subcaptionbox{\label{fig:non-convex-3rd-solution}
{\em non convex} (long time)
3rd solution \BALGO}
{\includegraphics[width=0.65\linewidth,height=0.65\linewidth]{non-convex-3rd-solution.pdf}}
\end{center}
\end{figure}
% end marc-simus.tex

==> Optimal UAV trajectory using HJB/marceau-simus-3.tex <==
% marceau-simus-3.tex %
%% A FAIRE : /21/09/2020
%% dans le tableau donner
%|p+-p-|-> cp  = critere d'arret sur p
%H+, H- -> cH  = critere d'arret sur H
%% rajouter 
%S1 = value function 1-phase marceau
% pour chaque cas (K, T2) -> show S1_phase
%%%%%%%%%%%%%
\begin{table}
\[
\hspace*{-6mm}
\begin{array}{|c c % xi R xi
c c c  %cP cH cB %new
c c c c % S H phi- phi+
| l % tau
%l %new
l |} % tau_0
\hline
\hline
R\ \xi  %new
%(\xi - \Delta) \times 10^4 &
& R\ \xi_0 %new
%(\xi_0 - \Delta) \times 10^4 & 
%|p^+ - p^-|
& c_P %new
& c_H  %H^+  %new
& c_B
& {\mathbf S}  & H^-  
& \phi^- & \phi^+  
& \tau  
%& T % new 
& \tau_0
%
%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{11}{|c|}
{\mathbf{K = 1}\ % t_0 = 0\ 
T = 0.1667\ 
\mbox{(long phase)}
\ra S_{1ph} = -0.0952 
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12) }
%%
\\
\myvec{51}{173.2} & %\myvec{55}{175}  % G-algo only
& 1.7\ 10^{-9}  % P+ - P- -> cP
& 0.2277 % cH !!
& 0.6104  %cB  %%% NEW -> after H- (=)H+
& -0.0971 %S 
& 0.8343 % H-
& 4.5296  & 0.2825 % phi- phi+
& 0.1432    %tau
%& 0.2500 %T new
& 0.0833 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 4)}
\\
\myvec{51}{173.2} & \myvec{55}{175} 
& 1.96\ 10^{-3} % cP
& 1.89\ 10^{-3} % cH  
&  0.0000 %cB % CHECK  
& -0.0971  %S
& 0.8343% H-
& 4.5297 & 0.2825 % phi- phi+
& 0.1432 % tau
& 0.1400 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\[1mm]
\hline
\hline
\multicolumn{11}{|c|}{K = 1\ t_0 = 0\ T = 0.0833  \mbox{ (short-phase)} 
\ra S_{1ph} =  -0.0347
}
\\[1mm]
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12) }
%%
\\
\myvec{49.6}{170.4} & % \myvec{48}{166}
& 1.98\ 10^{-9} %cP
& 0.4019 % cH
& 0.6104 % cB
& -0.0281 %S
&  0.8262  %H
& 1.8761 & 0.28894 % phi's
& 0.0593 % tau
 %&  0.1250  %new
 & 0.1200 %-> change 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 5)}
\\
 %%
\myvec{49.6}{170.4} & \myvec{48}{166} 
& 0.14 %cP
& 7.57\ 10^{-5}% cH
& 0.000 % cB % chec
& -0.0281 %S
&  0.8262  %H
& 1.8762 & 0.2889 % phi's
& 0.0593 % tau
 %&  0.1250  %new
 &  0.0580 % tau0
 %% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% K = 2  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[1mm]
\hline
\hline
% 11 -> 10 
\multicolumn{11}{|c|}{\mathbf{K = 2}\ t_0 = 0\ T = 0.1667\ \mbox{(long phase)}
\ra S_{1ph} =   -0.0857}
%
\\
%\hline
%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12) }
%%
\\
\myvec{50.6}{172.4} & %\myvec{55}{175}  % G-algo only
& .41\ 10^{-10 }  % P+ - P- -> cP
& 3.65\ 10^{-3}  % cH !!
& 0.6104  %cB  %%% NEW -> after H- (=)H+
&  -0.0799  % S 
& 0.8247 %% H-
& 2.9762  &  0.2859 % phi- phi+
& 0.1330   %tau
%& 0.2500 %T new
& %0.0833 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 4)}
%%
\\
\myvec{50.6}{172.4} & 
\myvec{40.}{160}  % G-algo only
& 4.03\ 10^{-3} % P+ - P- -> cP
& 4.28\ 10^{-4}  % cH !!
& 0.0000 %cB  %%% NEW -> after H- (=)H+
& -0.0799  % S 
& 0.8247 %% H-
& 2.9762 &  0.2859 % phi- phi+
& 0.1330   %tau
%& 0.2500 %T new
& 0.1300 %tau0
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
\\ %T = 0.0833 % -> DONE
\hline
\hline
\multicolumn{11}{|c|}{K = 2\ t_0 = 0\ T = 0.0833 \mbox{ (short-phase)}
\ra S_{1ph} =  -0.0193}
\\
%\hline
%%%%%% B-ALGO %%%%%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12) }
%%
\\
\myvec{47.7}{167.4} & %\myvec{4.}{164}  % G-algo only
& 1.7\ 10^{-9}  % P+ - P- -> cP
& 0.2277 % cH !!
& 0.6104  %cB  %%% NEW -> after H- (=)H+
& -0.102 %S 
& 0.9173 % H-
& 1.1419 &  0.2745 % phi- phi+
& 0.0510    %tau
%& 0.2500 %T new
& %0.0833 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 4)}
\\
\myvec{51}{173.2} & \myvec{55}{175} 
& 0.7123 % cP
&1.39\ 10^{-4} % cH  
&  0.0000 %cB % CHECK  
& -0.102 %S 
& 0.9173 % H-
& 1.1419 &  0.2745 % phi- phi+
& 0.0510    %tau
%& 0.2500 %T new
& 0.05 %tau0
%%%%%%%%%%%%%%%
\\
\hline
\end{array}
\]
\caption{\label{simus-marceau:table}
Table of results with 
%both 
\BALGO and \GRADALGO 
for 
K = 1, 2 %two values of mass $K$ 
and 
T = 0.1667 and 0.0833.
%of final time $T$.
\\
1 spatial unity corresponds approximatively to 11m.
Here final point is
$R\ z_T 
= (z_T - \Delta)* 1000. 
= (70, 164)$ % New
}
%+ associated scaling to do on impulsions
\end{table}
%%%%%%%%%%%%%%%%%%%%%%

==> Optimal UAV trajectory using HJB/marceau-simus-4.tex <==
% marceau-simus-4.tex %
% szT= [129.83 ; 155.56]
% K60 - T = 1200 and 1800
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{comment}
\begin{table}
\[
\hspace*{-8mm} % -6mm
\begin{array}{|c c % xi R xi
c c c  %cP cH cB %new
c c c c % S H phi- phi+
| l % tau
%l %new
l |} % tau_0
\hline
\hline
\vspace*{1mm}
%\bar{\xi}  %new
s\xi
%(\xi - \Delta) \times 10^4 &
& %\bar{\xi_0 }%new
s\xi_0
%(\xi_0 - \Delta) \times 10^4 & 
%|p^+ - p^-|
& c_P %new
& c_H  %H^+  %new
& c_B
& {\mathbf S}  & H^-  
& \phi^- & \phi^+  
& \tau  
%& T % new 
& \tau_0
%
%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{11}{|c|}
{\mathbf{K = 60}\ % t_0 = 0\ 
T = 1200
\ 
\mbox{(short phase)}
\ra S_{1ph} = -221.4103
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12) }
%%
\\
\myvec{53.76}{188.40} & % \bar{xi} %\myvec{55}{175}  % G-algo only
&  2.75\ 10^{-12}  % P+ - P- -> cP
&   0.0219     % cH !!
&  0.6104   %cB  %%% NEW -> after H- (=)H+
& -168.5713 %S 
&  0.8131 % H-
& 1.9803  & 0.9236 % phi- phi+
&538.69%63    %tau
%& 0.2500 %T new
& 600 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 5)}
\\
\myvec{53.76}{188.40} 
& \myvec{60}{200} 
& 0.7531 % cP
& 2.56\ 10^{-12} % cH  
&  0.0000 %cB % CHECK  
& -168.5713  %S
& 0.8131 % H-
& 1.9802 &  0.9237 % phi- phi+
& 538.68%34% tau
&300 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{11}{|c|}
{\mathbf{K = 60}\ % t_0 = 0\ 
T = 1800
\
\mbox{(long phase)}
\ra S_{1ph} = -637.9077
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12)}
%%
\\
\myvec{56.81}{192.70} & % \bar{xi} %\myvec{55}{175}  % G-algo only
& 7.54\ 10^{-12}  % P+ - P- -> cP
& 0.0598      % cH !!
& 0.6104   %cB  %%% NEW -> after H- (=)H+
& -641.6388  %S 
&  0.8332 % H-
& 4.1764  & 0.9273 % phi- phi+
&1136.09%62   %tau
%& 0.2500 %T new
& 900 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 2)}
\\
\myvec{56.81}{192.70} 
& \myvec{60}{180} 
& 7.58\ 10^{-6}  % cP
& 1.25\ 10^{-12} % cH  
&  0.0000 %cB % CHECK  
& -641.6388    %S
&  0.8332% H-
& 4.1763 & 0.9273 % phi- phi+
& 1136.08%59 % tau
& 1500 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{11}{|c|}
{\mathbf{K = 30 (* 1111.1111)^2}\ % t_0 = 0\ 
T = 1200
\
\mbox{(long phase)}
\ra S_{1ph} = -399.1474 
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12)}
%%
\\
\myvec{111.051}{13.173} & % \bar{xi} %\myvec{55}{175}  % G-algo only
& 4.21\ 10^{-9}  % P+ - P- -> cP
&  0.4613       % cH !!
& 0.6104   %cB  %%% NEW -> after H- (=)H+
& -393.1217  %S 
&   0.8313  % H-
&  3.7936 &  0.9289 % phi- phi+
& 729.71 %62   %tau
%& 0.2500 %T new
& ~900 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 2)}
\\
\myvec{11.051}{13.173} 
& \myvec{111.04}{13.16} % xi0 
& 0.0864   % cP
& 1.47\ 10^{-12} % cH  
&  0.0000 %cB % CHECK  
& -393.1217   %S
&   0.8313 % H-
&  3.7933 &  0.9290 % phi- phi+
& 729.65 %59 % tau
& 600 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\
\hline
\end{array}
\]
\caption{\label{simus-marceau4:table}
Table of results with 
%both 
\BALGO and \GRADALGO 
for 
$K = 60$
%two values of mass $K$ 
,
$T = 1200$ and $T = 1800$
(s)
\enspace.
%of final time $T$.
\\
1 spatial unity corresponds to %111.111m.
100m % CHECK
\enspace.
%\\CHECK
} % caption
\end{table}
%\end{comment}

==> Optimal UAV trajectory using HJB/marceau-simus-5.tex <==
% marceau-simus-5.tex %
% szT= [129.83 ; 155.56]
% K 30/60 * 1111.1111^2 
% - T = 1200 and 1800
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{comment}
\begin{table}
\[
\hspace*{-8mm} % -6mm
\begin{array}{|c c % xi R xi
c c c  %cP cH cB %new
c c c c % S H phi- phi+
| l % tau
%l %new
l |} % tau_0
\hline
\hline
\vspace*{1mm}
%\bar{\xi}  %new
%s
\xi
%(\xi - \Delta) \times 10^4 &
& %\bar{\xi_0 }%new
%s
\xi_0
%(\xi_0 - \Delta) \times 10^4 & 
%|p^+ - p^-|
& c_P %new
& c_H  %H^+  %new
& c_B
& {\mathbf S}  & H^-  
& \phi^- & \phi^+  
& \tau  
%& T % new 
& \tau_0
%
%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{11}{|c|}
{\mathbf{K = 60 * 1111.1111^2}\ % t_0 = 0\ 
T = 1200
\ 
\mbox{(short phase)}
\ra S_{1ph} = -221.4103
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12) }
%%
\\
%\myvec{53.76}{188.40} & %
\myvec{111.048%4
}{13.170}%13.1696
%\bar{xi-0} 
& ~
%\myvec{55}{175}  % G-algo only
&  2.75\ 10^{-12}  % P+ - P- -> cP
&   0.0219     % cH !!
&  0.6104   %cB  %%% NEW -> after H- (=)H+
& -168.5713 %S 
&  0.8131 % H-
& 1.9803  & 0.9236 % phi- phi+
&538.69%63    %tau
%& 0.2500 %T new
& 600 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 5)}
\\
%\myvec{53.76}{188.40}
\myvec{111.048%4
}{13.170}%.1696 
& %\myvec{60}{200}
\myvec{111.054}%0
{13.18}%0
& 0.7531 % cP
& 2.56\ 10^{-12} % cH  
&  0.0000 %cB % CHECK  
& -168.5713  %S
& 0.8131 % H-
& 1.9802 &  0.9237 % phi- phi+
& 538.68%34% tau
& 300 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{11}{|c|}
{\mathbf{K = 60
(* 1111.1111)^2}\ 
% t_0 = 0\ 
T = 1800
\
\mbox{(long phase)}
\ra S_{1ph} = -637.9077
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12)}
%%
\\
%\myvec{56.81}{192.70} 
\myvec{111.0511}{13.1734}
& % \bar{xi} %\myvec{55}{175}  % G-algo only
& 7.54\ 10^{-12}  % P+ - P- -> cP
& 0.0598      % cH !!
& 0.6104   %cB  %%% NEW -> after H- (=)H+
& -641.6388  %S 
&  0.8332 % H-
& 4.1764  & 0.9273 % phi- phi+
&1136.09%62   %tau
%& 0.2500 %T new
& 900 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 2)}
\\
%\myvec{56.81}{192.70} 
\myvec{111.0511}{13.1734}
& %\myvec{60}{180} 
\myvec{111.0540}{13.1620} 
& 7.58\ 10^{-6}  % cP
& 1.25\ 10^{-12} % cH  
&  0.0000 %cB % CHECK  
& -641.6388    %S
&  0.8332% H-
& 4.1763 & 0.9273 % phi- phi+
& 1136.08%59 % tau
& 1500 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{11}{|c|}
{\mathbf{K = 30 (* 1111.1111)^2}\ % t_0 = 0\ 
T = 1200
\
\mbox{(long phase)}
\ra S_{1ph} = -399.1474 
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12)}
%%
\\
\myvec{111.051}{13.173} & % \bar{xi} %\myvec{55}{175}  % G-algo only
& 4.21\ 10^{-9}  % P+ - P- -> cP
&  0.4613       % cH !!
& 0.6104   %cB  %%% NEW -> after H- (=)H+
& -393.1217  %S 
&   0.8313  % H-
&  3.7936 &  0.9289 % phi- phi+
& 729.71 %62   %tau
%& 0.2500 %T new
& ~900 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 2)}
\\
\myvec{11.051}{13.173} 
& \myvec{111.04}{13.16} % xi0 
& 0.0864   % cP
& 1.47\ 10^{-12} % cH  
&  0.0000 %cB % CHECK  
& -393.1217   %S
&   0.8313 % H-
&  3.7933 &  0.9290 % phi- phi+
& 729.65 %59 % tau
& 600 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\
\hline
\end{array}
\]
\caption{\label{simus-marceau4:table}
Table of results with 
%both 
\BALGO and \GRADALGO 
for 
$K = 60$
%two values of mass $K$ 
,
$T = 1200$ and $T = 1800$
(s)
\enspace.
%of final time $T$.
\\
1 spatial unity corresponds to %111.111m.
100m % CHECK
\enspace.
%\\CHECK
} % caption
\end{table}
%\end{comment}

==> Optimal UAV trajectory using HJB/marceau-simus-6.tex <==
% marceau-simus-6.tex %
% szT= [129.83 ; 155.56]
% K 30/60 * 1111.1111^2 
% - T = 1200 and 1800
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{comment}
\begin{table*}[t!] %[H]
\[
\hspace*{-8mm} % -6mm
\begin{array}{|c % c % xi xi0
%%%% c c c  %cP cH cB %new
c c c c % S H phi- phi+
| l % tau
%l %new
%l 
| % tau_0
} 
\hline
\hline
\vspace*{1mm}
%\bar{\xi}  %new
%s
\xi
%(\xi - \Delta) \times 10^4 &
% & \xi_0
%(\xi_0 - \Delta) \times 10^4 & 
%|p^+ - p^-|
%%%% & c_P %new
%%%% & c_H  %H^+  %new
%%%% & c_B
& {\mathbf S}  & H^-  
& \phi^- & \phi^+  
& \tau  
%& T % new 
% & \tau_0
%
%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
%% 11 -> 8
\multicolumn{6}{|c|}
{ \mathbf{a)}\ 
K = 60 \times r^2
%* 1111.1111^2
%}\ % t_0 = 0\ 
\enspace,
\ T = 1200
\ 
%\mbox{(short phase)}
\ra S_{1ph} = -221.4103
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{6}{|c|}{\BALGO\ (Niter = 12) }
%%
\\
%\myvec{53.76}{188.40} & %
\myvec{111.048%4
}{13.170}%13.1696
%\bar{xi0} 
%& %xi0
%\myvec{55}{175}  % G-algo only
%%% &  2.75\ 10^{-12}  % P+ - P- -> cP
%%%% &   0.0219     % cH !!
%%%% &  0.6104   %cB  %%% NEW -> after H- (=)H+
& -168.5713 %S 
&  0.8131 % H-
& 1.9803  & 0.9236 % phi- phi+
&538.69%63    %tau
%& 0.2500 %T new
% & 600 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{6}{|c|}{\GRADALGO (Niter = 5)}
\\
%\myvec{53.76}{188.40}
\myvec{111.048%4
}{13.170}%.1696 
% & %\myvec{60}{200} % xi0
%\myvec{111.054}{13.18} % xi0
%%%% & 0.7531 % cP
%%%% & 2.56\ 10^{-12} % cH  
%%%% &  0.0000 %cB % CHECK  
& -168.5713  %S
& 0.8131 % H-
& 1.9802 &  0.9237 % phi- phi+
& 538.68%34% tau
% & 300 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{6}{|c|}
{ \mathbf{b)}\
K = 60 \times r^2
%(* 1111.1111)^2
%}\ 
\enspace,
% t_0 = 0\
\ T = 1800
\
%\mbox{(long phase)}
\ra S_{1ph} = -637.9077
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{6}{|c|}{\BALGO\ (Niter = 12)}
%%
\\
%\myvec{56.81}{192.70} 
\myvec{111.0511}{13.1734}
%& %xi0
%\bar{xi} %\myvec{55}{175}  % G-algo only
%%%% & 7.54\ 10^{-12}  % P+ - P- -> cP
%%%% & 0.0598      % cH !!
%%%% & 0.6104   %cB  %%% NEW -> after H- (=)H+
& -641.6388  %S 
&  0.8332 % H-
& 4.1764  & 0.9273 % phi- phi+
&1136.09%62   %tau
%& 0.2500 %T new
% & 900 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{6}{|c|}{\GRADALGO (Niter = 2)}
\\
%\myvec{56.81}{192.70} 
\myvec{111.0511}{13.1734}
%& 
%\myvec{60}{180} 
%\myvec{111.0540}{13.1620}  % xi0
%%%% & 7.58\ 10^{-6}  % cP
%%%% & 1.25\ 10^{-12} % cH  
%%%% &  0.0000 %cB % CHECK  
& -641.6388    %S
&  0.8332% H-
& 4.1763 & 0.9273 % phi- phi+
& 1136.08%59 % tau
% & 1500 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{6}{|c|}
{ \mathbf{c)}\
K = 30 \times r^2
%(* 1111.1111)^2
%}\ % t_0 = 0\
\enspace,
\ T = 1200
\
%\mbox{(short phase)}
\ra S_{1ph} = -399.1474 
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{6}{|c|}{\BALGO\ (Niter = 12)}
%%
\\
\myvec{111.051}{13.173} 
% &  % xi0
% \bar{xi} %\myvec{55}{175}  % G-algo only
%%%% & 4.21\ 10^{-9}  % P+ - P- -> cP
%%%% &  0.4613       % cH !!
%%%% & 0.6104   %cB  %%% NEW -> after H- (=)H+
& -393.1217  %S 
&  0.8313  % H-
&  3.7936 & 0.9289 % phi- phi+
& 729.71 %62   %tau
%& 0.2500 %T new
% & ~900 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{6}{|c|}{\GRADALGO (Niter = 2)}
\\
\myvec{11.051}{13.173} 
%& \myvec{111.04}{13.16} % xi0 
%%%% & 0.0864   % cP
%%%% & 1.47\ 10^{-12} % cH  
%%%% &  0.0000 %cB % CHECK  
& -393.1217   %S
&   0.8313 % H-
&  3.7933 &  0.9290 % phi- phi+
& 729.65 %59 % tau
% & 600 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\
\hline
\end{array}
\]
\caption{\label{simus-marceau6:table}
Table of results with 
%both 
\BALGO\ and \GRADALGO 
for 
$K = 30, 60 \times r^2$
%two values of mass $K$ 
,
$T = 1200, 1800 s$
\\
%with
and
%of final time $T$.
$r = 
\frac{40 \times 10^6}{360 \times 100}
\approx 1111.1111$
(corresponding to scaled spatial unity of 100m).
\\
Also, $S_{1ph}$ denotes the total  single-phase cost
(\ie assuming only one, effective hotspot).
%\\CHECK
} % caption
\end{table*}
%\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% TABLE II lengths-speeds.
\begin{table*}[t!]%[t]
\[
\hspace*{-8mm} % -6mm
%\begin{array}{| l |  c c | c c | }
\begin{array}{|  l |  c c | c c  |}
\hline
\hline
%%%%%
\multicolumn{1}{| l |}
{case}
& %%%
\multicolumn{2}{ c |}
{\mbox{bi-phase}}
& %%% !!!!!
\multicolumn{2}{ c |}
{\mbox{single-phase}}
\\[1mm]
%\hline
%%%%%%
&
% !!
L\ (\mbox{km}) & \Vmean (\mbox{m/s})
& 
L\ (\mbox{km}) & \Vmean (\mbox{m/s})
\\
\hline
%%%%%
%%
 %1 & 2 & 3 & 4
 {\mathbf{a)}} 
 &
 12.41 & 10.34 
 &
 11.71 & 9.76 
%%%%%%%
\\[1mm]
\hline
%\\
{\mathbf{b)}} 
&
13.80 & 7.66 
 &
12.53 & 6.96
%%%%%%%%%%
\\[1mm]
\hline
%\multicolumn{4}{|c|}
%{\mathbf{c)}}
%\\
{\mathbf{c)}} 
&
13.64 & 11.37 
&
12.37 & 10.30 
\\
\hline
\end{array}
\]
\caption{\label{tab:length-speed} Table of trajectory lengths and related average speeds.}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
%%%%%%%% lengths 2 phases  %%%%%%
    \enspace:
    \\
    case (a) : $L = 12.41$ kms
     \enspace, 
     $\Vmean = 10.34$ m/s 
    \\
    case (b) : $L = 13.80$ kms
    \enspace,
    $\Vmean = 7.66$ m/s
    \\
    case (c) : $L = 13.64$ kms
    \enspace,
    $\Vmean = 11.37$ m/s
%    
%%%%% lengths 1 phase
a) K = 60 T = 1200
\ra L = 0.1054 
L = 11.71 km / V = 9.76 m/s
%
b) K = 60 T = 1800
\ra L = 0.1128 
L = 12.53 km / V = 6.96 m/s
%
c) K = 30 T = 1200
\ra L = 0.1113 
L = 12.37 km - V = 10.30 m/s\
\end{comment}
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% IN COMMENT %%%%%%%%%%%%%
\begin{comment}
\\
For %sake of commodity, 
better presentation,
we define 
the new origin
%the space vector
$\Delta = \MYSHIFT$
and scale the spatial results 
a
\begin{align*}
\xi \ra
s\xi = r\ (\xi - \Delta)
%\times 10^3
\enspace,
&  
\hspace*{20mm}
\mbox{with}
&
%%
\\[1mm]
%r = \frac{40000.}{360}
r = %\frac{40 \times 10^6}{360}
%\times \frac{1000.}{\mbox{unity}}
\times \frac{1.}{\mbox{unity}}
&
\hspace*{20mm} 
\mbox{unity} = 100\ (m)
\enspace, 
&
\ra r 
= \frac{4010^6}{100}
%\approx 1111.1111
\hspace*{20mm}
%
%\\
%R = r\ .* \mbox{diag} (\ \mbox{cosd}\ (zh_1(2))\ ,  1.\ ) 
\end{align*}
\end{comment}
%%%%%% END  COMMENT %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% RESULTS AND COMMENTS %%%%%\\
%%%%%%%%%%%%%%%%%%%%%%%%
% corrected
\begin{comment}
In the example presented here,
$z_T = (111.12 , 13.14)$
\enspace,
yielding
$sz_T = (129.83, 155.56)$
\enspace.
%%%%%% estimation 
\\
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Optimal UAV trajectory using HJB/marceau-simus.tex <==
% marceau-simus.tex %
%%%%%%%%%%%%%
\begin{table}
\[
\hspace*{-6mm}
\begin{array}{|c c c c c c c c | l l l |}
\hline
\hline
\xi - \Delta & \xi_0 - \Delta & |p^+ - p^-|
& S  &  H^-  & H^+  & \phi^- &  \phi^+ &  
\tau  & T %t2 
&\tau_0
%
\\
\hline
\hline
\multicolumn{11}{|c|}{\mathbf{K = 2}\ t_0 = 0\ T = 0.25\ \mbox{(long phase)}}
%
\\
%\hline
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 4) }
%%
\\
\myvec{0.0471}{0.1666} & \myvec{0.0441}{0.1632} & 0.0000
& -0.1705  & 0.8348  & 0.8347 &  5.4568  & 0.0518 &  
0.2439  & 0.2500 &
\\
\hline
%%%%%%%%  GRAD- ALGO
\multicolumn{11}{|c|}{\GRADALGO Niter = 5}
\\    
\myvec{0.0471}{0.1666} & \myvec{0.0400}{0.1600} & 0.0000 
&-0.1705  & 0.8348   &0.8348   &5.4568  & 0.0517 &  
0.2439 &  0.2500 &  0.2400
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
\hline
\hline
\multicolumn{11}{|c|}{K = 2\ t_0 = 0\ T = 0.125 \mbox{ (short-phase)} }
\\
%\hline
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO (Niter = 4) }
\\
%%
\myvec{0.0468 }{0.1663} &\myvec{0.0441}{0.1632} &   0.0000 
& -0.0677  & 0.7986 &  0.7986 & 2.6543 &  0.0540 & 
0.1186 &  0.1250  & 0.0625 
%
\\
\hline
\multicolumn{11}{|c|}{\GRADALGO (Niter = 4)}
%
\\    
 \myvec{0.0468}{0.1663} & \myvec{0.0400}{0.1600} &  0.0001 
 & -0.0677 &  0.7986 &  0.7987 &  2.6543  & 0.0540 &
 0.1186 &  0.1250 &  0.1100 
%%%%%%%%%%%%%
%%%%%%%%%%%%%
\\
\hline
\hline
\hline
\multicolumn{11}{|c|}{\mathbf{K = 1}\ t_0 = 0\ T = 0.25\ \mbox{(long phase)}}
\\
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 4) }
%%
\\
\myvec{0.0471}{0.1666} & \myvec{0.0400}{0.1600} & 0.0000 
 &-0.1819  & 0.8376 &  0.8376 &  7.7740  & 0.0515 & 
 0.2457  & 0.2500  & 0.1200 
%% 
\\
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 4)}
\\
%
\myvec{0.0471}{0.1666} & \myvec{0.0400}{0.1600} & 0.0000 
 & -0.1819 &  0.8376 &  0.8376  & 7.7739 &  0.0516  & 0.2457 &   0.2500   & 0.1200 
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\
\hline
\hline
\multicolumn{11}{|c|}{K = 1\ t_0 = 0\ T = 0.125 \mbox{ (short-phase)} }
\\
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 4) }
%%
\\
\myvec{0.0470}{0.1665}  & \myvec{0.0400}{0.1600} & 0.0000 
 & -0.0776 &  0.8228 &  0.8229  & 3.8170 &  0.0524 &  
 0.1206 &  0.1250  & 0.1200 
 %% 
\\
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 5)}
\\
 %%
\myvec{0.0470}{0.1665} & \myvec{0.0400}{0.1600} &  0.0000 &
 -0.0776 & 0.8228 & 0.8228 & 3.8169  & 0.0524 &  
 0.1206 &  0.1250 &  0.1200
\\
\hline
\end{array}
\]
\caption{\label{simus-marceau:table}
Table of results with both \BALGO and \GRADALGO 
for two values of mass and of final time.}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%


==> Optimal UAV trajectory using HJB/marceau-simus2.tex <==
% marceau-simus2.tex %
%% A FAIRE : /21/09/2020
%% dans le tableau donner
%|p+-p-|-> cp  = critere d'arret sur p
%H+, H- -> cH  = critere d'arret sur H
%% rajouter 
%S1 = value function 1-phase marceau
% pour chaque cas (K, T2) -> show S1_phase
%%%%%%%%%%%%%
\begin{table}
\[
\hspace*{-6mm}
\begin{array}{|c c c c c c c c | l l l |}
\hline
\hline
(\xi - \Delta) \times 10^4 & 
(\xi_0 - \Delta) \times 10^4 & 
|p^+ - p^-|
& S  &  H^-  & H^+  & \phi^- &  \phi^+ &  
\tau  & T %t2 
&\tau_0
%
\\
\hline
\hline
\multicolumn{11}{|c|}{\mathbf{K = 2}\ t_0 = 0\ T = 0.25\ \mbox{(long phase)}}
%
\\
%\hline
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 4) }
%%
\\
\myvec{471}{1666} & \myvec{441}{632} & 0.0000
& -0.1705  & 0.8348  & 0.8347 &  5.4568  & 0.0518 &  
0.2439  & 0.2500 &
\\
\hline
%%%%%%%%  GRAD- ALGO
\multicolumn{11}{|c|}{\GRADALGO Niter = 5}
\\    
\myvec{471}{1666} & \myvec{400}{1600} & 0.0000 
&-0.1705  & 0.8348   &0.8348   &5.4568  & 0.0517 &  
0.2439 &  0.2500 &  0.2400
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
\hline
\hline
\multicolumn{11}{|c|}{K = 2\ t_0 = 0\ T = 0.125 \mbox{ (short-phase)} }
\\
%\hline
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO (Niter = 4) }
\\
%%
\myvec{468 }{1663} &\myvec{441}{1632} &   0.0000 
& -0.0677  & 0.7986 &  0.7986 & 2.6543 &  0.0540 & 
0.1186 &  0.1250  & 0.0625 
%
\\
\hline
\multicolumn{11}{|c|}{\GRADALGO (Niter = 4)}
%
\\    
 \myvec{468}{1663} & \myvec{400}{1600} &  0.0001 
 & -0.0677 &  0.7986 &  0.7987 &  2.6543  & 0.0540 &
 0.1186 &  0.1250 &  0.1100 
%%%%%%%%%%%%%
%%%%%%%%%%%%%
\\
\hline
\hline
\hline
\multicolumn{11}{|c|}{\mathbf{K = 1}\ t_0 = 0\ T = 0.25\ \mbox{(long phase)}}
\\
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 4) }
%%
\\
\myvec{471}{1666} & \myvec{400}{1600} & 0.0000 
 &-0.1819  & 0.8376 &  0.8376 &  7.7740  & 0.0515 & 
 0.2457  & 0.2500  & 0.1200 
%% 
\\
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 4)}
\\
%
\myvec{471}{1666} & \myvec{400}{1600} & 0.0000 
 & -0.1819 &  0.8376 &  0.8376  & 7.7739 &  0.0516  & 0.2457 &   0.2500   & 0.1200 
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\
\hline
\hline
\multicolumn{11}{|c|}{K = 1\ t_0 = 0\ T = 0.125 \mbox{ (short-phase)} }
\\
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 4) }
%%
\\
\myvec{470}{1665}  & \myvec{400}{1600} & 0.0000 
 & -0.0776 &  0.8228 &  0.8229  & 3.8170 &  0.0524 &  
 0.1206 &  0.1250  & 0.1200 
 %% 
\\
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 5)}
\\
 %%
\myvec{470}{1665} & \myvec{400}{1600} &  0.0000 &
 -0.0776 & 0.8228 & 0.8228 & 3.8169  & 0.0524 &  
 0.1206 &  0.1250 &  0.1200
\\
\hline
\end{array}
\]
\caption{\label{simus-marceau:table}
Table of results with 
%both 
\BALGO and \GRADALGO 
for two values of mass $K$ 
and of final time $T$.
\\
1 spatial unity corresponds approximatively to 11m.
Here final point is
$(z_T - \Delta)* 1000. = (50, 164)$ % New
}
%+ associated scaling to do on impulsions
\end{table}
%%%%%%%%%%%%%%%%%%%%%%

==> Optimal UAV trajectory using HJB/proof-gradient.tex <==
% proof-gradient.tex
\subsection{... proof .... gradient non-convergence}
\label{app:gradient-non-convergence-proof}
%Proof:
All the results come from the fact that 
the following terms
%$\alpha$,
%Hamiltonians $H^+, H^-$
%and $\det(H(ξ,τ))$
can be expressed as (affine), isotropic quadratic
forms \wrt $\xi$, 
with a {\bf positive} quadratic term.
%1st item: results from the closed form of 
%$\alpha$ for the bi-phase value function resulting %fro
\begin{itemize}
%%%%%
\item $\alpha$
\enspace: 
from Appendix 
\ref{app:geometrical-non-convexity-condition} %G
and Eq. \eqref{alpha=d2Sdt2:eq},
each phase coefficient $\alpha_i, i = 1, 2$
is a quadratic affine form \wrt $\xi$
expressing as
%\[
$
A_i\ {\parallel \xi \parallel}^2 + B_i \cdot \xi + C_i
%%
 \ \ 
\mbox { with quadratic coefficient }
A_i = K\ \dfrac{\omega_i^3 \cosh\phase_i}{\sinh \phase_i^3} 
> 0
%% for phase_i > 0 i.e. time admissibility conditions
$
\\
Thus same property holds for total coefficient $\alpha = \alpha_1 + \alpha_2$


%%%%%
\item $\det({\cal H}(\xi, \tau))$ 
\enspace: 
from Appendix
\ref{diagonal-hessian:app}
Eq. \eqref{eq:Hessian-second}
%%
\begin{align*}
D = 
\det({\cal H}(\xi, \tau))
&=
K\ h \cdot 
\left\{ 
K\ h\ \alpha - {\parallel \Pi  \parallel}^2
\right\}
&=
K h \cdot 
\left\{ 
K h (\alpha_1 + \alpha_2) - {\parallel \Pi_1 + \Pi_2 \parallel}^2
\right\}
\end{align*}
%%
In what follows we note
$
\{u_i\} = \sum_{i=1,2} u_i
$
\enspace.
Since $\Pi_i$ is a linear control in $\xi$ 
(and in the other coordinate), it appears
that $D$ has the quadratic form property required
with quadratic coefficient %wrt $\xi$ 
%%
\[
A = 
K^2 
\left[
\{ \omega_i \coth \phase_i\} 
\{
\dfrac{\omega_i^3 \cosh\phase_i}{\sinh \phase_i^3}
\}
- 
\{\dfrac{\omega_i^2}{\sinh^2\phase_i} \}^2
\right]
> 0
\]
from $\cosh \phase_i \geq 1$
and Schwarz-like inequality
\[
\{\frac{a_i^2}{\lambda_i} \} 
\{a_i^2\ \lambda_i\}
\geq 
\{ a_i^2 \}^2 
\enspace,
\mbox{ with }
\lambda_i = \frac{\omega_i}{\sinh\phase_i} > 0
\mbox{ and }
a_i =\lambda_i > 0
\enspace!
\]
\end{itemize}


==> alternating-descent-algorithm.tex <==
% alternating-descent-algorithm.tex
% ms 21.09.20

\subsection{An Alternating Optimization Algorithm}

We now study a time-independent bi-phase scenario, in which a trajectory from $z_0$ to $z_T$ crosses the interface at time $\tau$ and location $\xi$. We present an Alternating Optimization Algorithm (Algorithm~\ref{alg:aoa}) that provides a stationary trajectory in the sense of Theorem~\ref{th:multiphase}. The algorithm consists in alternatively optimizing $\tau$ (steps 9-17) and $\xi$ (steps 18-26) by using the results of Theorem~\ref{th:multiphase}. For every fixed $\tau$ and $\xi$, the current trajectory is the concatenation of the optimal trajectory between $(t_0,z_0)$ and $(\tau,\xi)$ and the optimal trajectory between $(\tau,\xi)$ and $(T,z_T)$ (step 27). Every iteration of the algorithm only requires the evaluation of two Hamiltonians or the computation of a point $B$, see \eqref{location-B-ms:eq}, and its projection on the interface. Therefore the complexity of an iteration is  $O(1)$. In simulations, MPC is used to produce an initial trajectory.

\def\HSPONE{z_{h1}} % HOTSPOT 1
\def\HSPTWO{z_{h2}} % HOTSPOT 2

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.8\linewidth]{mpc-vs-aoa}
\end{center}
\caption{\label{fig:mpc-vs-aoa}MPC trajectory and Alternating Optimization Algorithm trajectory with two hot spots.}
\end{figure} 

\begin{figure}[H]
\begin{center}
\includegraphics[width=0.8\linewidth]{costfunction-scenario4}
\end{center}
\caption{\label{fig:costfunction-tau-scenario4}Cost function along the iterations of the Alternating Optimization Algorithm trajectory.}
\end{figure}



MPC
This projection is performed in steps 19-20 of the algorithm.


Figure~\ref{fig:mpc-vs-aoa} shows the MPC trajectory and the trajectory obtained from Algorithm~\ref{alg:aoa} after 60 iterations in a bi-phase landscape. The traffic intensity is shown in three dimensions in Figure~\ref{fig:systemmodel}: It is a bi-phase landscape made of two hot-spots, where the peak of traffic in $z_{h2}$ is higher than in $z_{h1}$. The Alternating Optimization Algorithm has gradually moved the interface crossing time and location in order to spend more time in the second hot-spot and to go closer to $z_{h2}$. 
Figure~\ref{fig:costfunction-tau-scenario4} shows how the cost function has decreased along the iterations and thus how our algorithm has improved over the MPC solution. From iterations 1 to 45, $\tau$ has been gradually updated; at iteration 46, $\xi$ is updated once; $\xi$ is again updated once at iteration 59.
%
\begin{comment}
In Figure~\ref{fig:potentialenergy-speed-scenario4} (top), we see how the difference between the potential energy before and after the interface tends to zero. Figure~\ref{fig:potentialenergy-speed-scenario4} (bottom) shows the difference between the velocity vectors before and after crossing the interface. On the resulting stationary trajectory, velocity is continuous on the interface.  
\end{comment}



\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%
\begin{algorithm}%[H]
\caption{Alternating Optimization Algorithm}\label{alg:aoa}
\begin{algorithmic}[1]
\State {\bf Input:} $t_0$, $T$, $z_0$, $z_T$, $z_{h1}$, $z_{h2}$, $u_{01}$, $u_{02}$, $\omega_1$, $\omega_2$, $u_{11}$,  $u_{12}$, an initial trajectory $z(t)$, the initial crossing time and position $(\tau, \xi)\in [\tau;T]\times \mathcal{I}$, $\delta \tau>0$, $\epsilon_{\tau}>0$, $\epsilon_{\xi}>0$, $\epsilon_{S}>0$.
\State {\bf Output:} $(\tau, \xi)\in [\tau;T]\times \mathcal{I}$  such that the conditions of Theorem~\ref{th:multiphase}
\State $\tau'\gets \tau$; $\xi'\gets \xi$
\State $\texttt{timenotfound} \gets 1$; $\texttt{positionnotfound} \gets 0$
\State $\{z(t)\}_{t_0\leq t\leq T}\gets $ an initial feasible trajectory, e.g. from MPC
\State Compute $S$ along $\{z(t)\}_{t_0\leq t\leq T}$
\Do
	\State $S'\gets S$
	\If{$\texttt{timenotfound}$}
		\State Compute $H_1$ and $H_2$ at $(\tau, \xi)$ according to (\ref{Hamilton-Jacobi-backward-ms:eq}-\ref{Hamilton-Jacobi-forward-ms:eq})
		\State $\tau \gets \tau + sign(H_1-H_2)\delta \tau$
		\If{$|\tau'-\tau|<\epsilon_{\tau}$}
			\State $\texttt{timenotfound}\gets 0$
			\State $\texttt{positionnotfound} \gets 1$
		\EndIf
		\State $\tau'\gets \tau$
	\EndIf
	\If{$\texttt{positionnotfound}$}
		\State Compute $B$ according to (\ref{location-B-ms:eq})
		\State $\xi \gets proj_{\mathcal{I}}(B)$, see (\ref{algo-proj-B:eq}) %$\nabla_{\xi} S=h(\xi-B)$
		\If{$||\xi'-\xi||<\epsilon_{\xi}$}
			\State $\texttt{timenotfound}\gets 1$
			\State $\texttt{positionnotfound} \gets 0$
		\EndIf
		\State $\xi'\gets \xi$
	\EndIf
    \State $\{z(t)\}_{t_0\leq t \leq T}\gets \texttt{OPTTRAJ}(z_{h1}, u_{01}, u_{11}, \omega_1, z_0, t_0,$ $\xi, \tau) \cup \texttt{OPTTRAJ}(z_{h2}, u_{02}, u_{12}, \omega_2, \xi, \tau, z_T, T)$  (\texttt{OPTTRAJ} provides optimal trajectory using \eqref{eq:trajhotspot},\eqref{eq:ellipse})
    %see \texttt{OPTTRAJ} function in Algorithm~\ref{alg:mpc})
    \State Cd{comment}ompute $S$ for $\{z(t)\}_{t_0\leq t\leq T}$ according to (\ref{eq:vu0neg}) 
\doWhile{$|S'-S|>\epsilon_S$}
\end{algorithmic}
\end{algorithm}



\begin{comment}
\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{potentialenergy-speed-scenario4v2}
\end{center}
\caption{\label{fig:potentialenergy-speed-scenario4}Alternating Optimization Algorithm trajectory: (top) $H_1-H_2$: Difference in potential energy before and after crossing the interface; (bottom) $||a_1-a_2||$: Norm of the difference of velocity vectors before and after crossing the interface.}
\end{figure}
\end{comment}

==> gradient-convergence.tex <==
% gradient-convergence.tex
%% to insert in 
%\section{Algoritms}
%\paragraph{Procedure for seeking an optimal $\tau$ given a fixed  $\xi$}
%\\
However
the following "non-convergence" results hold \textcolor{red}{MC: on a supposé que le drone traversait l'interface entre t0 et T non ? Sinon on se ramène au cas d'une seule interface, non ?}
%%%%
\begin{lemma}
\label{lem:outside-time-limits}
\eqref{h-coefficient:eq}:
Consider
$g(\tau)$ in ..
%\omega_1\, \coth(\omega_1(\tau -t_0)) + \omega_2\, \coth(\omega_2(T - \tau))$
Then
\\
%\begin{itemize}
%\item
in the case where 
$\omega_2 > \omega_1$ % check
then
$g(\tau)$ is {\bf negative} for $\tau > T$
(and also in $[t_0 - \epsilon, t_0[$)
%\item
\\
in the case where 
$\omega_1 > \omega_2$ % check
then
$g(\tau)$ is {\bf negative} for $\tau < t_0$
((and also in $]T, T + \epsilon]$)
%\end{itemize}
\end{lemma}
Proof: easy.
%\\
Thus if $\tau \notin ]t_0, T[$
the total value function could be non-convex. %% TO CHECK

\begin{theorem}
\label{th:gradient-non-convergence}
Consider current time value
$\tau \in ]t_0, T[$
and total Hessian
\eqref{eq:Hessian-second}.
%of the value function.
%\eqref{eq:Hessian-second}.
Then
\begin{itemize}
%
\item
the locus of points $\xi$
such that 
$\alpha 
= {\cal H}_{33}(\xi, \tau)
= \frac{d^2S}{d\tau^2}
< 0$
%in 
%\eqref{eq:Hessian-second}
%of the value function
is either empty
or a {\bf disk}
(inside of a {\bf circle})
\item the locus of points
such that
$\det({\cal H}(\xi, \tau)) < 0$
is either empty
or 
a {\bf disk}
%% the inside of a {\bf circle}
%
%% NOT SURE HERE-> CHECK
\begin{comment}
\item  
now consider time updating %%$\tau$:
$\tau \ra \tau + \delta \tau$ by a standard Newton-type method.
\\
%Then 
The locus of points $\xi$ such that
$\tau + \delta \tau 
\notin\ ]t_0, T[$
is the intersection two {\bf disks}
(possibly empty)
%either empty or a {\bf circular crown}
\end{comment}
%%
\end{itemize}
\end{theorem}
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Proof in Appendix
\ref{app:gradient-non-convergence-proof}
%%% PROOFS  %
\input{proof-gradient.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% RESULTS %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\\[1mm]
Influence of initial time $\tau_0$
associated "non-convergence basin" of starting points
$\xi_0$
in the \GRADALGO
are shown in in Figs
\ref{fig:marceau-non-convex1}
and
\ref{fig:marceau-non-convex2}.
%\\
In this example,
$z_T = (111.07, 13.164)$
%yielding
,
$szT = (77.78, 182.22)$ 
.
We select
$K=20, T = 800$
and the \BALGO optimal solution is 
$\xi^* = (56.65, 192.35)$ 
and 
$\tau^* = 683.15$
\enspace.

%%%%%%%%%%%%%%%%%%%
%%% FIGURES %%%%
%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\begin{subfigure}[t]{0.5\textwidth}
\centering
%
\includegraphics[width=1.\textwidth]{tau600-K20-T800.pdf}
\caption{$\tau = 600$
(close to solution) }
\label{fig:marceau-non-convex1}
\end{subfigure}
%
%~
\begin{subfigure}[t]
{0.5\textwidth}
\centering
\includegraphics[width=1.\textwidth]{tau400-K20-T800.pdf}
\caption{$\tau = 400$ 
(far from solution) }
\label{fig:marceau-non-convex2}
\end{subfigure}
%\caption{test}
\caption{
%$K = 20 - T = 800$%
Each subfigure 
shows spatial non-convergence basins for $\xi$
,
for two values of $\tau$.
}
\end{figure}




==> marc-simus.tex <==
% marc-simus.tex

Drone initial conditions 
as well as
network simulation parameters are shown in
Table \ref{parameters:table}.
%\\
\begin{table}[h!]
\[
\begin{array}{| c c c c  | c c c c | c c c c |}
% 14 items
\hline
\multicolumn{4}{| c |}{\mbox{general}}
& % test !!
\multicolumn{4}{c |}{\mbox{zone 1}} % ok !!
&
\multicolumn{4}{c|}{\mbox{zone 2}}
\\
\hline
z_0 & z_T 
%& z_{h1} & z_{h2} 
& t_0 & T  
%%
& z_h & u_0 & u_1 & \w
%
& z_h & u_0 & u_1 & \w
%%%%%
\\ 
\hline
\hline
%%%%%% CONVEX CASE %%%%%%%%%
\multicolumn{12}{| c |}{convex\ case}
\\
\hline
%%% numerical values %%%
-1\ -1 & 10\ 10 %& 5\ 1 & 6\ 8.5 
& 0 & 2.2
%%
& 5\ 1 & 2.645 & 20 & 1.627
%
& 6\ 8.5 &  8.265 & 40 & 2.875
%%%%%
\\
\hline
\hline
%%%%%% NON-CONVEX CASE %%%%%%%%%
\multicolumn{12}{| c |}{non-convex\ case}
\\
\hline
10\ 5 & 10\ 6 
%& z_{h1} & z_{h2} 
& 0 & 3.6 
%%
& 2\ -2  & 1.6327 & 20 & 1.2778
%
& 8\ 12 &  5.102 & 40  & 2.2588
\\
\hline
\end{array}
\]
\caption{Parameters used in 
experimental simulations.
$K = 1$ for all cases
\label{parameters:table}}
\end{table}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
Results are shown in Table \ref{results-grad-b-curve:table}.
%\\
%%%%%%%%%%%%%% TABLES SOLUTIONS %%%%%%%%%%%%
\begin{table}[h]%!] %% [h!] [h]ere overrides All other options
\[
\begin{array}{|c c c c c c c c | l l |}
\hline
\multicolumn{10}{|c|}
{\mbox{\em convex case}}
\\
\hline
%%
\xi & \norm{p^+ - p^-} & \hat{S} 
& |{\cal H}|
& H^+ & H^-  
& \tau &  T
& \mbox{ Solution} 
& % new
%%%%%%%%%%%%%%% CONVEX CASE %%%%%%%%%%%%%%%%%%%
\\[3mm]
\hline
\hline
 4.8481~5.3883 & 0.00981
& \mathbf{33.096 } 
& +
& 44.797  & 44.797  &  0.964  &   2.2
&
\GRADALGO
& % new
Fig.\ \ref{fig:convex-solution}
%%
\\[3mm]
\hline 
4.8456~5.3888 & 0.00000
& 33.096 
& +
&  44.801  & 44.797 & 0.9637 & 2.2
&
\BALGO & '' % new
%%%%%%%%%%%%%%%% NON-CONVEX CASE %%%%%%%%%%%%%%
\\[3mm]
\hline
\hline
\multicolumn{10}{|c|}
{\mbox{\em non-convex case}}
\\
\hline
6.3726~6.2484 & 0.00320 
& 100.32 
& -
& 10.773  & 10.773  & 2.6773  & 3.6
&
\mbox{n. 1 } \GRADALGO
&
Fig.\ \ref{fig:non-convex-1st-solution}
%%%%%
\\[3mm]
6.3733~6.2482 & 0.00000
& 100.32
& -
& 10.771  & 10.775 &  2.6771  &  3.6
&
\mbox{n. 1 } \BALGO
&
%[a,b]=[1,3]
''
%%%%%
\\[3mm]
9.8461~5.5062 & 0.0000
& \mathbf{-39.416} 
& +
& 39.881 & 39.862 & 0.035  & 3.6
& 
\mbox{n. 2 }\BALGO 
%% THE GOOD ONE !!
&
Fig.\ \ref{fig:non-convex-2nd-solution}
%%%%%
\\[3mm]
%\hline 
6.3302~6.3865 &  0.00180
& 78.338 
& +
&  16.123 &  16.123 & 3.5462  & 3.6
&
\mbox{n. 3 } \BALGO
&
Fig.\ \ref{fig:non-convex-3rd-solution}
\\[1mm]
\hline
%%%%%%%%%%%%%
\end{array}
\]
%%
\caption{\label{results-grad-b-curve:table}
Table of results with both gradient and the $B-$curve algorithms}
\end{table}
%%%%%%%
%~\\
Some remarks on the results:
\begin{enumerate}
\item the \GRADALGO and the dichotomic \BALGO 
with initial search interval
$[a, b] = [t_0, T]$
coincide
to the same %numerical 
optimum $(\xi^*, \tau^*)$ 
for the {\em convex} simulation case
(less that $3.\ e^-3$ on $\tau^*$)
\enspace.
%%
\item the \GRADALGO and the dichotomic \BALGO 
with initial search interval
$[a, b] = [1.,3.]$)
coincide
to the same %numerical 
optimum $(\xi^*, \tau^*)$ 
for the {\em non-convex} simulation case: 
(about $2.\ e^-4$ on $\tau^*$)
\enspace.
%
\item 
The two other (local) optimal solutions for this non-convex case
(including the global optimum, namely  $\#2$) are only attained by the \BALGO.
\item a note on local eigenvalues sign
: possible non-convexity (saddle point)
\end{enumerate}
%%
%%%%%%%%%%%%%% FIGURES SOLUTIONS %%%%%%%%%%%%
\begin{figure}[h!] %% [h!] [h]ere overrides All other options ?
\begin{center}
\subcaptionbox{\label{fig:convex-solution}
{\em convex case} (short time)  solution \GRADALGO}
{\includegraphics[width=0.65\linewidth,height=0.65\linewidth]{convex-case-solution.pdf}}
%%
\subcaptionbox{\label{fig:non-convex-1st-solution}
{\em non convex} (long time) 1st solution \GRADALGO}
{\includegraphics[width=0.65\linewidth,height=0.65\linewidth]{non-convex-1st-solution.pdf}}
\end{center}
%\caption{
\end{figure}
%%%%%%%%%%%
%%%%%%%%%%
\begin{figure}[h!] %% [h!] [h]ere overrides All other options ?
\begin{center}
\subcaptionbox{\label{fig:non-convex-2nd-solution}
{\em non convex} (long time) {\bf 2nd solution} algo-B .}
{\includegraphics[width=0.65\linewidth,height=0.65\linewidth]{non-convex-2nd-solution.pdf}}
%%
\subcaptionbox{\label{fig:non-convex-3rd-solution}
{\em non convex} (long time)
3rd solution \BALGO}
{\includegraphics[width=0.65\linewidth,height=0.65\linewidth]{non-convex-3rd-solution.pdf}}
\end{center}
\end{figure}
% end marc-simus.tex

==> marceau-simus-3.tex <==
% marceau-simus-3.tex %
%% A FAIRE : /21/09/2020
%% dans le tableau donner
%|p+-p-|-> cp  = critere d'arret sur p
%H+, H- -> cH  = critere d'arret sur H
%% rajouter 
%S1 = value function 1-phase marceau
% pour chaque cas (K, T2) -> show S1_phase
%%%%%%%%%%%%%
\begin{table}
\[
\hspace*{-6mm}
\begin{array}{|c c % xi R xi
c c c  %cP cH cB %new
c c c c % S H phi- phi+
| l % tau
%l %new
l |} % tau_0
\hline
\hline
R\ \xi  %new
%(\xi - \Delta) \times 10^4 &
& R\ \xi_0 %new
%(\xi_0 - \Delta) \times 10^4 & 
%|p^+ - p^-|
& c_P %new
& c_H  %H^+  %new
& c_B
& {\mathbf S}  & H^-  
& \phi^- & \phi^+  
& \tau  
%& T % new 
& \tau_0
%
%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{11}{|c|}
{\mathbf{K = 1}\ % t_0 = 0\ 
T = 0.1667\ 
\mbox{(long phase)}
\ra S_{1ph} = -0.0952 
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12) }
%%
\\
\myvec{51}{173.2} & %\myvec{55}{175}  % G-algo only
& 1.7\ 10^{-9}  % P+ - P- -> cP
& 0.2277 % cH !!
& 0.6104  %cB  %%% NEW -> after H- (=)H+
& -0.0971 %S 
& 0.8343 % H-
& 4.5296  & 0.2825 % phi- phi+
& 0.1432    %tau
%& 0.2500 %T new
& 0.0833 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 4)}
\\
\myvec{51}{173.2} & \myvec{55}{175} 
& 1.96\ 10^{-3} % cP
& 1.89\ 10^{-3} % cH  
&  0.0000 %cB % CHECK  
& -0.0971  %S
& 0.8343% H-
& 4.5297 & 0.2825 % phi- phi+
& 0.1432 % tau
& 0.1400 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\[1mm]
\hline
\hline
\multicolumn{11}{|c|}{K = 1\ t_0 = 0\ T = 0.0833  \mbox{ (short-phase)} 
\ra S_{1ph} =  -0.0347
}
\\[1mm]
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12) }
%%
\\
\myvec{49.6}{170.4} & % \myvec{48}{166}
& 1.98\ 10^{-9} %cP
& 0.4019 % cH
& 0.6104 % cB
& -0.0281 %S
&  0.8262  %H
& 1.8761 & 0.28894 % phi's
& 0.0593 % tau
 %&  0.1250  %new
 & 0.1200 %-> change 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 5)}
\\
 %%
\myvec{49.6}{170.4} & \myvec{48}{166} 
& 0.14 %cP
& 7.57\ 10^{-5}% cH
& 0.000 % cB % chec
& -0.0281 %S
&  0.8262  %H
& 1.8762 & 0.2889 % phi's
& 0.0593 % tau
 %&  0.1250  %new
 &  0.0580 % tau0
 %% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% K = 2  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[1mm]
\hline
\hline
% 11 -> 10 
\multicolumn{11}{|c|}{\mathbf{K = 2}\ t_0 = 0\ T = 0.1667\ \mbox{(long phase)}
\ra S_{1ph} =   -0.0857}
%
\\
%\hline
%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12) }
%%
\\
\myvec{50.6}{172.4} & %\myvec{55}{175}  % G-algo only
& .41\ 10^{-10 }  % P+ - P- -> cP
& 3.65\ 10^{-3}  % cH !!
& 0.6104  %cB  %%% NEW -> after H- (=)H+
&  -0.0799  % S 
& 0.8247 %% H-
& 2.9762  &  0.2859 % phi- phi+
& 0.1330   %tau
%& 0.2500 %T new
& %0.0833 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 4)}
%%
\\
\myvec{50.6}{172.4} & 
\myvec{40.}{160}  % G-algo only
& 4.03\ 10^{-3} % P+ - P- -> cP
& 4.28\ 10^{-4}  % cH !!
& 0.0000 %cB  %%% NEW -> after H- (=)H+
& -0.0799  % S 
& 0.8247 %% H-
& 2.9762 &  0.2859 % phi- phi+
& 0.1330   %tau
%& 0.2500 %T new
& 0.1300 %tau0
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
\\ %T = 0.0833 % -> DONE
\hline
\hline
\multicolumn{11}{|c|}{K = 2\ t_0 = 0\ T = 0.0833 \mbox{ (short-phase)}
\ra S_{1ph} =  -0.0193}
\\
%\hline
%%%%%% B-ALGO %%%%%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12) }
%%
\\
\myvec{47.7}{167.4} & %\myvec{4.}{164}  % G-algo only
& 1.7\ 10^{-9}  % P+ - P- -> cP
& 0.2277 % cH !!
& 0.6104  %cB  %%% NEW -> after H- (=)H+
& -0.102 %S 
& 0.9173 % H-
& 1.1419 &  0.2745 % phi- phi+
& 0.0510    %tau
%& 0.2500 %T new
& %0.0833 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 4)}
\\
\myvec{51}{173.2} & \myvec{55}{175} 
& 0.7123 % cP
&1.39\ 10^{-4} % cH  
&  0.0000 %cB % CHECK  
& -0.102 %S 
& 0.9173 % H-
& 1.1419 &  0.2745 % phi- phi+
& 0.0510    %tau
%& 0.2500 %T new
& 0.05 %tau0
%%%%%%%%%%%%%%%
\\
\hline
\end{array}
\]
\caption{\label{simus-marceau:table}
Table of results with 
%both 
\BALGO and \GRADALGO 
for 
K = 1, 2 %two values of mass $K$ 
and 
T = 0.1667 and 0.0833.
%of final time $T$.
\\
1 spatial unity corresponds approximatively to 11m.
Here final point is
$R\ z_T 
= (z_T - \Delta)* 1000. 
= (70, 164)$ % New
}
%+ associated scaling to do on impulsions
\end{table}
%%%%%%%%%%%%%%%%%%%%%%

==> marceau-simus-4.tex <==
% marceau-simus-4.tex %
% szT= [129.83 ; 155.56]
% K60 - T = 1200 and 1800
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{comment}
\begin{table}
\[
\hspace*{-8mm} % -6mm
\begin{array}{|c c % xi R xi
c c c  %cP cH cB %new
c c c c % S H phi- phi+
| l % tau
%l %new
l |} % tau_0
\hline
\hline
\vspace*{1mm}
%\bar{\xi}  %new
s\xi
%(\xi - \Delta) \times 10^4 &
& %\bar{\xi_0 }%new
s\xi_0
%(\xi_0 - \Delta) \times 10^4 & 
%|p^+ - p^-|
& c_P %new
& c_H  %H^+  %new
& c_B
& {\mathbf S}  & H^-  
& \phi^- & \phi^+  
& \tau  
%& T % new 
& \tau_0
%
%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{11}{|c|}
{\mathbf{K = 60}\ % t_0 = 0\ 
T = 1200
\ 
\mbox{(short phase)}
\ra S_{1ph} = -221.4103
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12) }
%%
\\
\myvec{53.76}{188.40} & % \bar{xi} %\myvec{55}{175}  % G-algo only
&  2.75\ 10^{-12}  % P+ - P- -> cP
&   0.0219     % cH !!
&  0.6104   %cB  %%% NEW -> after H- (=)H+
& -168.5713 %S 
&  0.8131 % H-
& 1.9803  & 0.9236 % phi- phi+
&538.69%63    %tau
%& 0.2500 %T new
& 600 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 5)}
\\
\myvec{53.76}{188.40} 
& \myvec{60}{200} 
& 0.7531 % cP
& 2.56\ 10^{-12} % cH  
&  0.0000 %cB % CHECK  
& -168.5713  %S
& 0.8131 % H-
& 1.9802 &  0.9237 % phi- phi+
& 538.68%34% tau
&300 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{11}{|c|}
{\mathbf{K = 60}\ % t_0 = 0\ 
T = 1800
\
\mbox{(long phase)}
\ra S_{1ph} = -637.9077
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12)}
%%
\\
\myvec{56.81}{192.70} & % \bar{xi} %\myvec{55}{175}  % G-algo only
& 7.54\ 10^{-12}  % P+ - P- -> cP
& 0.0598      % cH !!
& 0.6104   %cB  %%% NEW -> after H- (=)H+
& -641.6388  %S 
&  0.8332 % H-
& 4.1764  & 0.9273 % phi- phi+
&1136.09%62   %tau
%& 0.2500 %T new
& 900 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 2)}
\\
\myvec{56.81}{192.70} 
& \myvec{60}{180} 
& 7.58\ 10^{-6}  % cP
& 1.25\ 10^{-12} % cH  
&  0.0000 %cB % CHECK  
& -641.6388    %S
&  0.8332% H-
& 4.1763 & 0.9273 % phi- phi+
& 1136.08%59 % tau
& 1500 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{11}{|c|}
{\mathbf{K = 30 (* 1111.1111)^2}\ % t_0 = 0\ 
T = 1200
\
\mbox{(long phase)}
\ra S_{1ph} = -399.1474 
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12)}
%%
\\
\myvec{111.051}{13.173} & % \bar{xi} %\myvec{55}{175}  % G-algo only
& 4.21\ 10^{-9}  % P+ - P- -> cP
&  0.4613       % cH !!
& 0.6104   %cB  %%% NEW -> after H- (=)H+
& -393.1217  %S 
&   0.8313  % H-
&  3.7936 &  0.9289 % phi- phi+
& 729.71 %62   %tau
%& 0.2500 %T new
& ~900 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 2)}
\\
\myvec{11.051}{13.173} 
& \myvec{111.04}{13.16} % xi0 
& 0.0864   % cP
& 1.47\ 10^{-12} % cH  
&  0.0000 %cB % CHECK  
& -393.1217   %S
&   0.8313 % H-
&  3.7933 &  0.9290 % phi- phi+
& 729.65 %59 % tau
& 600 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\
\hline
\end{array}
\]
\caption{\label{simus-marceau4:table}
Table of results with 
%both 
\BALGO and \GRADALGO 
for 
$K = 60$
%two values of mass $K$ 
,
$T = 1200$ and $T = 1800$
(s)
\enspace.
%of final time $T$.
\\
1 spatial unity corresponds to %111.111m.
100m % CHECK
\enspace.
%\\CHECK
} % caption
\end{table}
%\end{comment}

==> marceau-simus-5.tex <==
% marceau-simus-5.tex %
% szT= [129.83 ; 155.56]
% K 30/60 * 1111.1111^2 
% - T = 1200 and 1800
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{comment}
\begin{table}
\[
\hspace*{-8mm} % -6mm
\begin{array}{|c c % xi R xi
c c c  %cP cH cB %new
c c c c % S H phi- phi+
| l % tau
%l %new
l |} % tau_0
\hline
\hline
\vspace*{1mm}
%\bar{\xi}  %new
%s
\xi
%(\xi - \Delta) \times 10^4 &
& %\bar{\xi_0 }%new
%s
\xi_0
%(\xi_0 - \Delta) \times 10^4 & 
%|p^+ - p^-|
& c_P %new
& c_H  %H^+  %new
& c_B
& {\mathbf S}  & H^-  
& \phi^- & \phi^+  
& \tau  
%& T % new 
& \tau_0
%
%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{11}{|c|}
{\mathbf{K = 60 * 1111.1111^2}\ % t_0 = 0\ 
T = 1200
\ 
\mbox{(short phase)}
\ra S_{1ph} = -221.4103
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12) }
%%
\\
%\myvec{53.76}{188.40} & %
\myvec{111.048%4
}{13.170}%13.1696
%\bar{xi-0} 
& ~
%\myvec{55}{175}  % G-algo only
&  2.75\ 10^{-12}  % P+ - P- -> cP
&   0.0219     % cH !!
&  0.6104   %cB  %%% NEW -> after H- (=)H+
& -168.5713 %S 
&  0.8131 % H-
& 1.9803  & 0.9236 % phi- phi+
&538.69%63    %tau
%& 0.2500 %T new
& 600 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 5)}
\\
%\myvec{53.76}{188.40}
\myvec{111.048%4
}{13.170}%.1696 
& %\myvec{60}{200}
\myvec{111.054}%0
{13.18}%0
& 0.7531 % cP
& 2.56\ 10^{-12} % cH  
&  0.0000 %cB % CHECK  
& -168.5713  %S
& 0.8131 % H-
& 1.9802 &  0.9237 % phi- phi+
& 538.68%34% tau
& 300 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{11}{|c|}
{\mathbf{K = 60
(* 1111.1111)^2}\ 
% t_0 = 0\ 
T = 1800
\
\mbox{(long phase)}
\ra S_{1ph} = -637.9077
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12)}
%%
\\
%\myvec{56.81}{192.70} 
\myvec{111.0511}{13.1734}
& % \bar{xi} %\myvec{55}{175}  % G-algo only
& 7.54\ 10^{-12}  % P+ - P- -> cP
& 0.0598      % cH !!
& 0.6104   %cB  %%% NEW -> after H- (=)H+
& -641.6388  %S 
&  0.8332 % H-
& 4.1764  & 0.9273 % phi- phi+
&1136.09%62   %tau
%& 0.2500 %T new
& 900 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 2)}
\\
%\myvec{56.81}{192.70} 
\myvec{111.0511}{13.1734}
& %\myvec{60}{180} 
\myvec{111.0540}{13.1620} 
& 7.58\ 10^{-6}  % cP
& 1.25\ 10^{-12} % cH  
&  0.0000 %cB % CHECK  
& -641.6388    %S
&  0.8332% H-
& 4.1763 & 0.9273 % phi- phi+
& 1136.08%59 % tau
& 1500 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
\hline
\hline
%\hline
\multicolumn{11}{|c|}
{\mathbf{K = 30 (* 1111.1111)^2}\ % t_0 = 0\ 
T = 1200
\
\mbox{(long phase)}
\ra S_{1ph} = -399.1474 
}
\\[1mm]
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 12)}
%%
\\
\myvec{111.051}{13.173} & % \bar{xi} %\myvec{55}{175}  % G-algo only
& 4.21\ 10^{-9}  % P+ - P- -> cP
&  0.4613       % cH !!
& 0.6104   %cB  %%% NEW -> after H- (=)H+
& -393.1217  %S 
&   0.8313  % H-
&  3.7936 &  0.9289 % phi- phi+
& 729.71 %62   %tau
%& 0.2500 %T new
& ~900 %tau0
%% 
\\[1mm]
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 2)}
\\
\myvec{11.051}{13.173} 
& \myvec{111.04}{13.16} % xi0 
& 0.0864   % cP
& 1.47\ 10^{-12} % cH  
&  0.0000 %cB % CHECK  
& -393.1217   %S
&   0.8313 % H-
&  3.7933 &  0.9290 % phi- phi+
& 729.65 %59 % tau
& 600 % tau0
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\
\hline
\end{array}
\]
\caption{\label{simus-marceau4:table}
Table of results with 
%both 
\BALGO and \GRADALGO 
for 
$K = 60$
%two values of mass $K$ 
,
$T = 1200$ and $T = 1800$
(s)
\enspace.
%of final time $T$.
\\
1 spatial unity corresponds to %111.111m.
100m % CHECK
\enspace.
%\\CHECK
} % caption
\end{table}
%\end{comment}

==> marceau-simus.tex <==
% marceau-simus.tex %
%%%%%%%%%%%%%
\begin{table}
\[
\hspace*{-6mm}
\begin{array}{|c c c c c c c c | l l l |}
\hline
\hline
\xi - \Delta & \xi_0 - \Delta & |p^+ - p^-|
& S  &  H^-  & H^+  & \phi^- &  \phi^+ &  
\tau  & T %t2 
&\tau_0
%
\\
\hline
\hline
\multicolumn{11}{|c|}{\mathbf{K = 2}\ t_0 = 0\ T = 0.25\ \mbox{(long phase)}}
%
\\
%\hline
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 4) }
%%
\\
\myvec{0.0471}{0.1666} & \myvec{0.0441}{0.1632} & 0.0000
& -0.1705  & 0.8348  & 0.8347 &  5.4568  & 0.0518 &  
0.2439  & 0.2500 &
\\
\hline
%%%%%%%%  GRAD- ALGO
\multicolumn{11}{|c|}{\GRADALGO Niter = 5}
\\    
\myvec{0.0471}{0.1666} & \myvec{0.0400}{0.1600} & 0.0000 
&-0.1705  & 0.8348   &0.8348   &5.4568  & 0.0517 &  
0.2439 &  0.2500 &  0.2400
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
\hline
\hline
\multicolumn{11}{|c|}{K = 2\ t_0 = 0\ T = 0.125 \mbox{ (short-phase)} }
\\
%\hline
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO (Niter = 4) }
\\
%%
\myvec{0.0468 }{0.1663} &\myvec{0.0441}{0.1632} &   0.0000 
& -0.0677  & 0.7986 &  0.7986 & 2.6543 &  0.0540 & 
0.1186 &  0.1250  & 0.0625 
%
\\
\hline
\multicolumn{11}{|c|}{\GRADALGO (Niter = 4)}
%
\\    
 \myvec{0.0468}{0.1663} & \myvec{0.0400}{0.1600} &  0.0001 
 & -0.0677 &  0.7986 &  0.7987 &  2.6543  & 0.0540 &
 0.1186 &  0.1250 &  0.1100 
%%%%%%%%%%%%%
%%%%%%%%%%%%%
\\
\hline
\hline
\hline
\multicolumn{11}{|c|}{\mathbf{K = 1}\ t_0 = 0\ T = 0.25\ \mbox{(long phase)}}
\\
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 4) }
%%
\\
\myvec{0.0471}{0.1666} & \myvec{0.0400}{0.1600} & 0.0000 
 &-0.1819  & 0.8376 &  0.8376 &  7.7740  & 0.0515 & 
 0.2457  & 0.2500  & 0.1200 
%% 
\\
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 4)}
\\
%
\myvec{0.0471}{0.1666} & \myvec{0.0400}{0.1600} & 0.0000 
 & -0.1819 &  0.8376 &  0.8376  & 7.7739 &  0.0516  & 0.2457 &   0.2500   & 0.1200 
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\
\hline
\hline
\multicolumn{11}{|c|}{K = 1\ t_0 = 0\ T = 0.125 \mbox{ (short-phase)} }
\\
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 4) }
%%
\\
\myvec{0.0470}{0.1665}  & \myvec{0.0400}{0.1600} & 0.0000 
 & -0.0776 &  0.8228 &  0.8229  & 3.8170 &  0.0524 &  
 0.1206 &  0.1250  & 0.1200 
 %% 
\\
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 5)}
\\
 %%
\myvec{0.0470}{0.1665} & \myvec{0.0400}{0.1600} &  0.0000 &
 -0.0776 & 0.8228 & 0.8228 & 3.8169  & 0.0524 &  
 0.1206 &  0.1250 &  0.1200
\\
\hline
\end{array}
\]
\caption{\label{simus-marceau:table}
Table of results with both \BALGO and \GRADALGO 
for two values of mass and of final time.}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%


==> marceau-simus2.tex <==
% marceau-simus2.tex %
%% A FAIRE : /21/09/2020
%% dans le tableau donner
%|p+-p-|-> cp  = critere d'arret sur p
%H+, H- -> cH  = critere d'arret sur H
%% rajouter 
%S1 = value function 1-phase marceau
% pour chaque cas (K, T2) -> show S1_phase
%%%%%%%%%%%%%
\begin{table}
\[
\hspace*{-6mm}
\begin{array}{|c c c c c c c c | l l l |}
\hline
\hline
(\xi - \Delta) \times 10^4 & 
(\xi_0 - \Delta) \times 10^4 & 
|p^+ - p^-|
& S  &  H^-  & H^+  & \phi^- &  \phi^+ &  
\tau  & T %t2 
&\tau_0
%
\\
\hline
\hline
\multicolumn{11}{|c|}{\mathbf{K = 2}\ t_0 = 0\ T = 0.25\ \mbox{(long phase)}}
%
\\
%\hline
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 4) }
%%
\\
\myvec{471}{1666} & \myvec{441}{632} & 0.0000
& -0.1705  & 0.8348  & 0.8347 &  5.4568  & 0.0518 &  
0.2439  & 0.2500 &
\\
\hline
%%%%%%%%  GRAD- ALGO
\multicolumn{11}{|c|}{\GRADALGO Niter = 5}
\\    
\myvec{471}{1666} & \myvec{400}{1600} & 0.0000 
&-0.1705  & 0.8348   &0.8348   &5.4568  & 0.0517 &  
0.2439 &  0.2500 &  0.2400
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
\hline
\hline
\multicolumn{11}{|c|}{K = 2\ t_0 = 0\ T = 0.125 \mbox{ (short-phase)} }
\\
%\hline
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO (Niter = 4) }
\\
%%
\myvec{468 }{1663} &\myvec{441}{1632} &   0.0000 
& -0.0677  & 0.7986 &  0.7986 & 2.6543 &  0.0540 & 
0.1186 &  0.1250  & 0.0625 
%
\\
\hline
\multicolumn{11}{|c|}{\GRADALGO (Niter = 4)}
%
\\    
 \myvec{468}{1663} & \myvec{400}{1600} &  0.0001 
 & -0.0677 &  0.7986 &  0.7987 &  2.6543  & 0.0540 &
 0.1186 &  0.1250 &  0.1100 
%%%%%%%%%%%%%
%%%%%%%%%%%%%
\\
\hline
\hline
\hline
\multicolumn{11}{|c|}{\mathbf{K = 1}\ t_0 = 0\ T = 0.25\ \mbox{(long phase)}}
\\
%%%%
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 4) }
%%
\\
\myvec{471}{1666} & \myvec{400}{1600} & 0.0000 
 &-0.1819  & 0.8376 &  0.8376 &  7.7740  & 0.0515 & 
 0.2457  & 0.2500  & 0.1200 
%% 
\\
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 4)}
\\
%
\myvec{471}{1666} & \myvec{400}{1600} & 0.0000 
 & -0.1819 &  0.8376 &  0.8376  & 7.7739 &  0.0516  & 0.2457 &   0.2500   & 0.1200 
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\\
\hline
\hline
\multicolumn{11}{|c|}{K = 1\ t_0 = 0\ T = 0.125 \mbox{ (short-phase)} }
\\
%%%%%% B-ALGO %%%%
\multicolumn{11}{|c|}{\BALGO\ (Niter = 4) }
%%
\\
\myvec{470}{1665}  & \myvec{400}{1600} & 0.0000 
 & -0.0776 &  0.8228 &  0.8229  & 3.8170 &  0.0524 &  
 0.1206 &  0.1250  & 0.1200 
 %% 
\\
\hline
%%%%%%%%  GRAD- ALGO 
\multicolumn{11}{|c|}{\GRADALGO (Niter = 5)}
\\
 %%
\myvec{470}{1665} & \myvec{400}{1600} &  0.0000 &
 -0.0776 & 0.8228 & 0.8228 & 3.8169  & 0.0524 &  
 0.1206 &  0.1250 &  0.1200
\\
\hline
\end{array}
\]
\caption{\label{simus-marceau:table}
Table of results with 
%both 
\BALGO and \GRADALGO 
for two values of mass $K$ 
and of final time $T$.
\\
1 spatial unity corresponds approximatively to 11m.
Here final point is
$(z_T - \Delta)* 1000. = (50, 164)$ % New
}
%+ associated scaling to do on impulsions
\end{table}
%%%%%%%%%%%%%%%%%%%%%%

==> proof-gradient.tex <==
% proof-gradient.tex
\subsection{... proof .... gradient non-convergence}
\label{app:gradient-non-convergence-proof}
%Proof:
All the results come from the fact that 
the following terms
%$\alpha$,
%Hamiltonians $H^+, H^-$
%and $\det(H(ξ,τ))$
can be expressed as (affine), isotropic quadratic
forms \wrt $\xi$, 
with a {\bf positive} quadratic term.
%1st item: results from the closed form of 
%$\alpha$ for the bi-phase value function resulting %fro
\begin{itemize}
%%%%%
\item $\alpha$
\enspace: 
from Appendix 
\ref{app:geometrical-non-convexity-condition} %G
and Eq. \eqref{alpha=d2Sdt2:eq},
each phase coefficient $\alpha_i, i = 1, 2$
is a quadratic affine form \wrt $\xi$
expressing as
%\[
$
A_i\ {\parallel \xi \parallel}^2 + B_i \cdot \xi + C_i
%%
 \ \ 
\mbox { with quadratic coefficient }
A_i = K\ \dfrac{\omega_i^3 \cosh\phase_i}{\sinh \phase_i^3} 
> 0
%% for phase_i > 0 i.e. time admissibility conditions
$
\\
Thus same property holds for total coefficient $\alpha = \alpha_1 + \alpha_2$


%%%%%
\item $\det({\cal H}(\xi, \tau))$ 
\enspace: 
from Appendix
\ref{diagonal-hessian:app}
Eq. \eqref{eq:Hessian-second}
%%
\begin{align*}
D = 
\det({\cal H}(\xi, \tau))
&=
K\ h \cdot 
\left\{ 
K\ h\ \alpha - {\parallel \Pi  \parallel}^2
\right\}
&=
K h \cdot 
\left\{ 
K h (\alpha_1 + \alpha_2) - {\parallel \Pi_1 + \Pi_2 \parallel}^2
\right\}
\end{align*}
%%
In what follows we note
$
\{u_i\} = \sum_{i=1,2} u_i
$
\enspace.
Since $\Pi_i$ is a linear control in $\xi$ 
(and in the other coordinate), it appears
that $D$ has the quadratic form property required
with quadratic coefficient %wrt $\xi$ 
%%
\[
A = 
K^2 
\left[
\{ \omega_i \coth \phase_i\} 
\{
\dfrac{\omega_i^3 \cosh\phase_i}{\sinh \phase_i^3}
\}
- 
\{\dfrac{\omega_i^2}{\sinh^2\phase_i} \}^2
\right]
> 0
\]
from $\cosh \phase_i \geq 1$
and Schwarz-like inequality
\[
\{\frac{a_i^2}{\lambda_i} \} 
\{a_i^2\ \lambda_i\}
\geq 
\{ a_i^2 \}^2 
\enspace,
\mbox{ with }
\lambda_i = \frac{\omega_i}{\sinh\phase_i} > 0
\mbox{ and }
a_i =\lambda_i > 0
\enspace!
\]
\end{itemize}

